Decentralized Online Convex Optimization in Networked Systems

We study the problem of networked online convex optimization, where each agent individually decides on an action at every time step and agents cooperatively seek to minimize the total global cost over a finite horizon. The global cost is made up of three types of local costs: convex node costs, temporal interaction costs, and spatial interaction costs. In deciding their individual action at each time, an agent has access to predictions of local cost functions for the next $k$ time steps in an $r$-hop neighborhood. Our work proposes a novel online algorithm, Localized Predictive Control (LPC), which generalizes predictive control to multi-agent systems. We show that LPC achieves a competitive ratio of $1 + \tilde{O}(\rho_T^k) + \tilde{O}(\rho_S^r)$ in an adversarial setting, where $\rho_T$ and $\rho_S$ are constants in $(0, 1)$ that increase with the relative strength of temporal and spatial interaction costs, respectively. This is the first competitive ratio bound on decentralized predictive control for networked online convex optimization. Further, we show that the dependence on $k$ and $r$ in our results is near optimal by lower bounding the competitive ratio of any decentralized online algorithm.

==> Figures/information_structure.tex <==
\begin{tikzpicture}
\draw[draw=orange!50!white, line width=1.5pt, dashed] (40pt, 10pt) -- (40pt, 60pt);
\draw[draw=orange!50!white, line width=1.5pt] (40pt, 60pt) -- (40pt, 110pt);
\draw[draw=orange!50!white, line width=1.5pt, dashed] (120pt, 10pt) -- (120pt, 60pt);
\draw[draw=orange!50!white, line width=1.5pt] (120pt, 60pt) -- (120pt, 110pt);

\begin{scope}
    \draw[draw=black, line width=1pt, densely dashed] (0pt, 0pt) circle (5pt); 
    \node at (10pt, -10pt) {\footnotesize $u_1$};
    
    \draw[draw=black, line width=1pt, densely dashed] (40pt, 10pt) circle (5pt); 
    \node at (45pt, 20pt) {\footnotesize $u_2$};
    
    \draw[draw=black, line width=1pt, densely dashed] (80pt, 0pt) circle (5pt); 
    \node at (85pt, -10pt) {\footnotesize $v$};
    
    \draw[draw=black, line width=1pt, densely dashed] (120pt, 10pt) circle (5pt); 
    \node at (125pt, 20pt) {\footnotesize $u_3$};
    
    \draw[draw=black, line width=1pt, densely dashed] (160pt, 0pt) circle (5pt); 
    \node at (170pt, -10pt) {\footnotesize $u_4$};
    
    \draw[draw=blue!50!white, line width=1.5pt, dashed] (0pt, 0pt) -- (40pt, 10pt);
    \draw[draw=blue!50!white, line width=1.5pt, dashed] (40pt, 10pt) -- (80pt, 0pt);
    %\draw[draw=blue!50!white, line width=1.5pt] (0pt, 0pt) -- (80pt, 0pt);
    \draw[draw=blue!50!white, line width=1.5pt, dashed] (120pt, 10pt) -- (40pt, 10pt);
    \draw[draw=blue!50!white, line width=1.5pt, dashed] (80pt, 0pt) -- (120pt, 10pt);
    \draw[draw=blue!50!white, line width=1.5pt, dashed] (120pt, 10pt) -- (160pt, 0pt);
    %\draw[draw=blue!50!white, line width=1.5pt] (80pt, 0pt) -- (160pt, 0pt);
    
    \node at (-20pt, 0pt) {\footnotesize $t + 2$};
\end{scope}

\begin{scope}[yshift=50pt]
    \draw[draw=black, line width=1pt, densely dashed] (0pt, 0pt) circle (5pt); 
    \node at (10pt, -10pt) {\footnotesize $u_1$};
    
    \draw[draw=black, line width=1pt] (40pt, 10pt) circle (5pt); 
    \node at (45pt, 20pt) {\footnotesize $u_2$};
    
    \draw[draw=black, line width=1pt] (80pt, 0pt) circle (5pt); 
    \node at (85pt, -10pt) {\footnotesize $v$};
    
    \draw[draw=black, line width=1pt] (120pt, 10pt) circle (5pt); 
    \node at (125pt, 20pt) {\footnotesize $u_3$};
    
    \draw[draw=black, line width=1pt, densely dashed] (160pt, 0pt) circle (5pt); 
    \node at (170pt, -10pt) {\footnotesize $u_4$};
    
    \draw[draw=blue!50!white, line width=1.5pt, dashed] (0pt, 0pt) -- (40pt, 10pt);
    \draw[draw=blue!50!white, line width=1.5pt] (40pt, 10pt) -- (80pt, 0pt);
    %\draw[draw=blue!50!white, line width=1.5pt] (0pt, 0pt) -- (80pt, 0pt);
    \draw[draw=blue!50!white, line width=1.5pt] (120pt, 10pt) -- (40pt, 10pt);
    \draw[draw=blue!50!white, line width=1.5pt] (80pt, 0pt) -- (120pt, 10pt);
    \draw[draw=blue!50!white, line width=1.5pt, dashed] (120pt, 10pt) -- (160pt, 0pt);
    %\draw[draw=blue!50!white, line width=1.5pt] (80pt, 0pt) -- (160pt, 0pt);
    
    \node at (-20pt, 0pt) {\footnotesize $t + 1$};
\end{scope}

\begin{scope}[yshift=100pt]
    \draw[draw=black, line width=1pt, densely dashed] (0pt, 0pt) circle (5pt); 
    \node at (10pt, -10pt) {\footnotesize $u_1$};
    
    \draw[draw=black, line width=1pt] (40pt, 10pt) circle (5pt); 
    \node at (45pt, 20pt) {\footnotesize $u_2$};
    
    \draw[draw=black, line width=1pt] (80pt, 0pt) circle (5pt); 
    \node at (85pt, -10pt) {\footnotesize $v$};
    
    \draw[draw=black, line width=1pt] (120pt, 10pt) circle (5pt); 
    \node at (125pt, 20pt) {\footnotesize $u_3$};
    
    \draw[draw=black, line width=1pt, densely dashed] (160pt, 0pt) circle (5pt); 
    \node at (170pt, -10pt) {\footnotesize $u_4$};
    
    \draw[draw=blue!50!white, line width=1.5pt, dashed] (0pt, 0pt) -- (40pt, 10pt);
    \draw[draw=blue!50!white, line width=1.5pt] (40pt, 10pt) -- (80pt, 0pt);
    %\draw[draw=blue!50!white, line width=1.5pt] (0pt, 0pt) -- (80pt, 0pt);
    \draw[draw=blue!50!white, line width=1.5pt] (120pt, 10pt) -- (40pt, 10pt);
    \draw[draw=blue!50!white, line width=1.5pt] (80pt, 0pt) -- (120pt, 10pt);
    \draw[draw=blue!50!white, line width=1.5pt, dashed] (120pt, 10pt) -- (160pt, 0pt);
    %\draw[draw=blue!50!white, line width=1.5pt] (80pt, 0pt) -- (160pt, 0pt);
    
    \node at (-20pt, 0pt) {\footnotesize $t$};
\end{scope}

\draw[draw=orange!50!white, line width=1.5pt, dashed] (0pt, 0pt) -- (0pt, 100pt);
\draw[draw=orange!50!white, line width=1.5pt, dashed] (80pt, 0pt) -- (80pt, 50pt);
\draw[draw=orange!50!white, line width=1.5pt] (80pt, 50pt) -- (80pt, 100pt);
\draw[draw=orange!50!white, line width=1.5pt, dashed] (160pt, 0pt) -- (160pt, 100pt);
\end{tikzpicture}

==> Figures/regroup_decision_vars_pts.tex <==
\begin{tikzpicture}

\draw[draw=orange!50!white, line width=1.5pt] (40pt, 10pt) -- (40pt, 110pt);
\draw[draw=orange!50!white, line width=1.5pt] (120pt, 10pt) -- (120pt, 110pt);
\draw[draw=orange!50!white, line width=1.5pt] (0pt, 0pt) -- (0pt, 100pt);
\draw[draw=orange!50!white, line width=1.5pt] (80pt, 0pt) -- (80pt, 100pt);
\draw[draw=orange!50!white, line width=1.5pt] (160pt, 0pt) -- (160pt, 100pt);

\begin{scope}
    \draw[draw=black, line width=1pt] (0pt, 0pt) circle (2pt); 
    \node at (0pt, -10pt) {\footnotesize $x_3^1$};
    
    \draw[draw=black, line width=1pt] (40pt, 10pt) circle (2pt); 
    \node at (40pt, 20pt) {\footnotesize $x_3^2$};
    
    \draw[draw=black, line width=1pt] (80pt, 0pt) circle (2pt); 
    \node at (80pt, -10pt) {\footnotesize $x_3^3$};
    
    \draw[draw=black, line width=1pt] (120pt, 10pt) circle (2pt); 
    \node at (120pt, 20pt) {\footnotesize $x_3^4$};
    
    \draw[draw=black, line width=1pt] (160pt, 0pt) circle (2pt); 
    \node at (160pt, -10pt) {\footnotesize $x_3^5$};
    
    \draw[draw=blue!50!white, line width=1.5pt] (0pt, 0pt) -- (40pt, 10pt);
    \draw[draw=blue!50!white, line width=1.5pt] (40pt, 10pt) -- (80pt, 0pt);
    %\draw[draw=blue!50!white, line width=1.5pt] (0pt, 0pt) -- (80pt, 0pt);
    \draw[draw=blue!50!white, line width=1.5pt] (120pt, 10pt) -- (40pt, 10pt);
    \draw[draw=blue!50!white, line width=1.5pt] (80pt, 0pt) -- (120pt, 10pt);
    \draw[draw=blue!50!white, line width=1.5pt] (120pt, 10pt) -- (160pt, 0pt);
    %\draw[draw=blue!50!white, line width=1.5pt] (80pt, 0pt) -- (160pt, 0pt);
    
    \node at (-20pt, 0pt) {\footnotesize $t = 3$};
\end{scope}

\begin{scope}[yshift=50pt]
    \draw[draw=black, line width=1pt] (0pt, 0pt) circle (2pt); 
    \node at (0pt, -10pt) {\footnotesize $x_2^1$};
    
    \draw[draw=black, line width=1pt] (40pt, 10pt) circle (2pt); 
    \node at (40pt, 20pt) {\footnotesize $x_2^2$};
    
    \draw[draw=black, line width=1pt] (80pt, 0pt) circle (2pt); 
    \node at (80pt, -10pt) {\footnotesize $x_2^3$};
    
    \draw[draw=black, line width=1pt] (120pt, 10pt) circle (2pt); 
    \node at (120pt, 20pt) {\footnotesize $x_2^4$};
    
    \draw[draw=black, line width=1pt] (160pt, 0pt) circle (2pt); 
    \node at (160pt, -10pt) {\footnotesize $x_2^5$};
    
    \draw[draw=blue!50!white, line width=1.5pt] (0pt, 0pt) -- (40pt, 10pt);
    \draw[draw=blue!50!white, line width=1.5pt] (40pt, 10pt) -- (80pt, 0pt);
    %\draw[draw=blue!50!white, line width=1.5pt] (0pt, 0pt) -- (80pt, 0pt);
    \draw[draw=blue!50!white, line width=1.5pt] (120pt, 10pt) -- (40pt, 10pt);
    \draw[draw=blue!50!white, line width=1.5pt] (80pt, 0pt) -- (120pt, 10pt);
    \draw[draw=blue!50!white, line width=1.5pt] (120pt, 10pt) -- (160pt, 0pt);
    %\draw[draw=blue!50!white, line width=1.5pt] (80pt, 0pt) -- (160pt, 0pt);
    
    \node at (-20pt, 0pt) {\footnotesize $t = 2$};
\end{scope}

\begin{scope}[yshift=100pt]
    \draw[draw=black, line width=1pt] (0pt, 0pt) circle (2pt); 
    \node at (0pt, -10pt) {\footnotesize $x_1^1$};
    
    \draw[draw=black, line width=1pt] (40pt, 10pt) circle (2pt); 
    \node at (40pt, 20pt) {\footnotesize $x_1^2$};
    
    \draw[draw=black, line width=1pt] (80pt, 0pt) circle (2pt); 
    \node at (80pt, -10pt) {\footnotesize $x_1^3$};
    
    \draw[draw=black, line width=1pt] (120pt, 10pt) circle (2pt); 
    \node at (120pt, 20pt) {\footnotesize $x_1^4$};
    
    \draw[draw=black, line width=1pt] (160pt, 0pt) circle (2pt); 
    \node at (160pt, -10pt) {\footnotesize $x_1^5$};
    
    \draw[draw=blue!50!white, line width=1.5pt] (0pt, 0pt) -- (40pt, 10pt);
    \draw[draw=blue!50!white, line width=1.5pt] (40pt, 10pt) -- (80pt, 0pt);
    %\draw[draw=blue!50!white, line width=1.5pt] (0pt, 0pt) -- (80pt, 0pt);
    \draw[draw=blue!50!white, line width=1.5pt] (120pt, 10pt) -- (40pt, 10pt);
    \draw[draw=blue!50!white, line width=1.5pt] (80pt, 0pt) -- (120pt, 10pt);
    \draw[draw=blue!50!white, line width=1.5pt] (120pt, 10pt) -- (160pt, 0pt);
    %\draw[draw=blue!50!white, line width=1.5pt] (80pt, 0pt) -- (160pt, 0pt);
    
    \node at (-20pt, 0pt) {\footnotesize $t = 1$};
\end{scope}


\end{tikzpicture}

==> Proofs/graph-induced-band-mat-inverse.tex <==
    We first prove the lemma for the the special case where $D = 0$. 
    
    For the case $\hat{d} \neq 0$, write $\hat{d} = \upsilon q/2 + \kappa$ for integers $\upsilon, \kappa$ satisfying $\upsilon \geq 0, 1 \leq \kappa \leq q/2$. Following the same approach as the proof of Proposition 2.2 in \cite{demko1984decay}, we see that there exists a polynomial $p_\upsilon$ of degree $\upsilon$, where
    \[\norm{A^{-1} - p_\upsilon(A)} \leq \frac{1}{a_0}\cdot \frac{\left(1 + \sqrt{cond(A)}\right)^2}{2cond(A)} \gamma^{\hat{d}}\leq C \gamma^{\hat{d}},\]
    where the last inequality holds because $cond(A) \geq 1$.
    
    Since $p_v$ has degree $v < \frac{2 \hat{d}}{q}$ and $A$ is graph-induced $q$-banded, the matrix $p_{\upsilon}(A)$ satisfies $\left(p_{\upsilon}(A)\right)_{i, j} = 0$ for any $i \in S_R$ and $j \in S_C$.
    We then obtain
    \[\norm{P} = \norm{\left(A^{-1}\right)_{S_R,S_C}} = \norm{\left(A^{-1} - p_{\upsilon}(A)\right)_{S_R,S_C}} \leq \norm{A^{-1} - p_{\upsilon}(A)} \leq C \gamma^{\hat{d}},\]
    due to the fact that the 2-norm of a submatrix cannot be larger than that of the original matrix.
        
    For the case $\hat{d} = 0$, as $\norm{P} = \norm{\left(A^{-1}\right)_{S_R, S_C}} \leq \norm{A^{-1}} = \frac{1}{a_0} \leq C$, the result trivially holds.
    
    Now we show the general case (where $D_i \succeq 0$ for $1 \le i \le n$) through a reduction to the special case. Define a positive definite matrix $N := (a_0 I + D) \in \mathbb{S}^{n\omega}$, and then define matrix $H \in \mathbb{S}^{n\omega}$ as
    \[H := N^{-\frac{1}{2}} (A + D) N^{-\frac{1}{2}}.\]
    We start by showing that $I \preceq H \preceq \frac{b_0}{a_0}\cdot I$. For any $x \in \mathbb{R}^{n\omega}$, we observe that
    \begin{align*}
        x^{\top} H x &= x^{\top} N^{-\frac{1}{2}}A N^{-\frac{1}{2}}x + x^{\top} N^{-\frac{1}{2}}D N^{-\frac{1}{2}}x\\
        &\geq x^{\top} N^{-\frac{1}{2}} a_0 I N^{-\frac{1}{2}}x + x^{\top} N^{-\frac{1}{2}}D N^{-\frac{1}{2}}x\\
        &= x^{\top} N^{-\frac{1}{2}} (a_0 I + D) N^{-\frac{1}{2}}x\\
        &= \norm{x}^2.
    \end{align*}
    For the other inequality, note that $0 \prec N^{-1} \preceq \frac{1}{a_0} \cdot I$, so we have
    \begin{align*}
        x^{\top} H x &= x^{\top} N^{-\frac{1}{2}}A N^{-\frac{1}{2}}x + x^{\top} N^{-\frac{1}{2}}D N^{-\frac{1}{2}}x\\
        &\leq x^{\top} N^{-\frac{1}{2}} b_0 I N^{-\frac{1}{2}}x + x^{\top} N^{-\frac{1}{2}}D N^{-\frac{1}{2}}x\\
        &= x^{\top} N^{-\frac{1}{2}} (a_0 I + D) N^{-\frac{1}{2}}x + (b_0 - a_0) x^{\top} N^{-1} x\\
        &\leq \norm{x}^2 + \frac{b_0 - a_0}{a_0} \cdot \norm{x}^2\\
        &= \frac{b_0}{a_0}\cdot \norm{x}^2.
    \end{align*}
    Thus $I \preceq H \preceq \frac{b_0}{a_0} \cdot I$, which gives $cond(H) \leq \frac{b_0}{a_0} = cond(A)$. Note that $H$ is also $q$-banded, so we can apply the result of the special case ($D_i = 0, i=1,\cdots,n$) to obtain that
    \[\norm{(H^{-1})_{S_R,S_C}} \leq 2 \gamma_H^{\hat{d}} \leq 2 \gamma^{\hat{d}},\]
    where $\gamma_H = \left(\frac{\sqrt{cond(H)} - 1}{\sqrt{cond(H)} + 1}\right)^{2/q} \leq \gamma$. Using this inequality, we conclude that
    \begin{align*}
        \norm{P} = \norm{((A + D)^{-1})_{S_R,S_C}} &= \norm{\left(N^{-\frac{1}{2}} H^{-1} N^{-\frac{1}{2}}\right)_{S_R,S_C}}\\
        &\leq \norm{(a_0 I + D_{S_R})^{-\frac{1}{2}}} \cdot \norm{(H^{-1})_{S_R,S_C}} \cdot \norm{(a_0 I + D_{S_C})^{-\frac{1}{2}}}\\
        &\leq \frac{1}{a_0}\norm{(H^{-1})_{S_R,S_C}}\\
        &\leq C \gamma^{\hat{d}}.
    \end{align*}
    Here we apply the fact that $\norm{(a_0 I + D_{S})^{-\frac{1}{2}}} \leq \frac{1}{\sqrt{a_0}}$ since $D_S \succeq 0$.

==> graph.tex <==
\begin{figure}[t]
    	\centering
    	\begin{tikzpicture}[scale=0.8]
    	\node[right] () at (-2,0) {$t=0$};
    	\node[circle, draw, red] (11) at (0,0) {};
    	\node[circle, draw, red] (12) at (2,0) {};
    	\node[circle, draw, red] (13) at (4,0) {};
    	\node[] () at (5.5,0) {...};
    	\node[circle, draw, red] (14) at (7,0) {};
    	\node[circle, draw, red] (15) at (9,0) {};
    	\node[right] () at (10,0) {$x_0$ given};
    	%
    	\node[right] () at (-2,-1) {$t=1$};
    	\node[circle, draw, red] (21) at (0,-1) {};
    	\node[circle, draw, red] (22) at (2,-1) {};
    	\node[circle, draw, red] (23) at (4,-1) {};
    	\node[] () at (5.5,-1) {...};
    	\node[circle, draw, red] (24) at (7,-1) {};
    	\node[circle, draw, red] (25) at (9,-1) {};
    	\node[right] () at (10,-1) {$x_1$ to be decided};
    	%
    	\node[right] () at (-2,-2) {$t=2$};
    	
    	\node[circle, draw,  dashed, red] (31) at (0,-2) {};
    	\node[circle, draw,  dashed, red] (32) at (2,-2) {};
    	\node[circle, draw,  dashed, red] (33) at (4,-2) {};
    	\node[] () at (5.5,-2) {...};
    	\node[circle, draw,  dashed, red] (34) at (7,-2) {};
    	\node[circle, draw,  dashed, red] (35) at (9,-2) {};
    	\node[right] () at (10,-2) {$x_2$ to be decided};
    	
    	%
    	%\node[] () at (0,.6) {$v_1$};
    	%\node[] () at (2,.6) {$v_2$};
    	%\node[] () at (4,.6) {$v_3$};
    	%\node[] () at (5.5,.6) {...};
    	%\node[] () at (7,.6) {$v_{m-1}$};
    	%\node[] () at (9,.6) {$v_m$};
    	%
    	\draw[solid, thick, blue] (11) -- (12);
    	\draw[solid, thick, blue] (12) -- (13);
    	\draw[solid, thick, blue] (14) -- (15);
    	\draw[solid, thick, blue] (21) -- (22);
    	\draw[solid, thick, blue] (22) -- (23);
    	\draw[solid, thick, blue] (24) -- (25);
    
    	\draw[solid, thick, dashed, blue] (31) -- (32);
    	\draw[solid, thick, dashed, blue] (32) -- (33);
    	\draw[solid, thick, dashed, blue] (34) -- (35);
    	%
    	\draw[solid,  thick, green!70!blue] (11) -- (21);
    	\draw[solid,  thick, dashed, green!70!blue] (31) -- (21);
    	\draw[solid,  thick, green!70!blue] (12) -- (22);
    	\draw[solid,  thick, dashed, green!70!blue] (32) -- (22);
    	\draw[solid,  thick, green!70!blue] (13) -- (23);
    	\draw[solid,  thick, dashed, green!70!blue] (33) -- (23);
    	\draw[solid,  thick, green!70!blue] (14) -- (24);
    	\draw[solid,  thick, dashed, green!70!blue] (34) -- (24);
    	\draw[solid,  thick, green!70!blue] (15) -- (25);
    	\draw[solid,  thick, dashed, green!70!blue] (35) -- (25);
    	
    	%
    	\draw[solid,  thick, blue] (13) -- (4.8,0);
    	\draw[solid,  thick, blue] (6.2,0) -- (14);
    	\draw[solid,  thick, blue] (23) -- (4.8,-1);
    	\draw[solid,  thick, blue] (6.2,-1) -- (24);
    	\draw[solid,  thick, dashed, blue] (33) -- (4.8,-2);
    	\draw[solid,  thick, dashed, blue] (6.2,-2) -- (34);
    	%
    	\end{tikzpicture}
    	\caption{Example with $G$ being the path graph}
    \end{figure}

==> second_perturbation.tex <==
\begin{theorem}\label{thm:networked-exp-decay-tight}
Recall the following notation $h(\gamma) \coloneqq \sup_{v \in \mathcal{V}} \abs{\partial N_v^{\gamma}}$.
Define $a = \sum_{\gamma \ge 0}(\frac{3}{4})^{\gamma} h(\gamma)$ and $\gamma_S = \frac{\sqrt{1 + \Delta \ell_S/\mu} - 1}{\sqrt{1 + \Delta \ell_S/\mu} + 1}$.  Suppose Assumption \ref{assump:costs-and-feasible-sets} holds,  $a < \infty$ and $\mu > \max\{8a\ell_T, \Delta \ell_S\}$. Then
 the exponentially decaying local perturbation bound holds with $C_1 = C_2 =  \max\{\frac{a}{2(1 - 4al_T/\mu)}, \frac{(\Delta l_S/\mu) a^2}{\gamma_S(1 - 4al_T/\mu)}\}$, and
\begin{align*}
    \rho_T = \frac{4a\ell_T}{\mu}, \quad
    \rho_S = 2\gamma_S.
\end{align*}
\end{theorem}
